Deep Depth Estimation from Visual-Inertial SLAM

This paper addresses the problem of learning to complete a scene's depth from sparse depth points and images of indoor scenes. Specifically, we study the case in which the sparse depth is computed from a visual-inertial simultaneous localization and mapping (VI-SLAM) system. The resulting point cloud has low density, it is noisy, and has non-uniform spatial distribution, as compared to the input from active depth sensors, e.g., LiDAR or Kinect. Since the VI-SLAM produces point clouds only over textured areas, we compensate for the missing depth of the low-texture surfaces by leveraging their planar structures and their surface normals which is an important intermediate representation. The pre-trained surface normal network, however, suffers from large performance degradation when there is a significant difference in the viewing direction (especially the roll angle) of the test image as compared to the trained ones. To address this limitation, we use the available gravity estimate from the VI-SLAM to warp the input image to the orientation prevailing in the training dataset. This results in a significant performance gain for the surface normal estimate, and thus the dense depth estimates. Finally, we show that our method outperforms other state-of-the-art approaches both on training (ScanNet and NYUv2) and testing (collected with Azure Kinect) datasets.

==> iros_2020_arxiv/tex/01_introduction.tex <==
\section{Introduction}

Determining the dense depth of a scene has important applications in augmented reality, motion planning, and 3D mapping. 
%
This is often achieved by employing depth sensors such as Kinect and LiDAR. 
%
Besides the high-cost, size, and power requirements of depth sensors, their measurements are either sparse (LiDAR) or unreliable at glossy, reflective, and far-distance surfaces (Kinect).
%
Recent research has shown that some of the limitations of depth sensors can be overcome by employing RGB images along with the strong contextual priors learned from large-scale datasets ($\simeq$ 200K images), using a deep convolutional neural network (CNN).
%
Specifically, to produce dense depth estimates, recent approaches have employed CNNs with three types of inputs: (a) a single RGB image (e.g.,~\cite{eigen2014depth, fu2018dorn, laina2016DeeperDepthPrediction, liu2015learning, li2018megadepth});
%~\cite{bloesch2018codeslam, weerasekera2017MonocularSN, eigen2014depth, fu2018dorn, laina2016DeeperDepthPrediction, liu2015learning, li2018megadepth, Liu2019planercnn, fei2019geosupervised};
%
(b) poses (position and orientation) and optical flow from multiple images (e.g.,~\cite{liu2019neuralrgbd, ummenhofer2017demon, zhou2018deeptam});
%
(c) a single RGB image and sparse depth~\cite{tang2019sparse2dense, liao2017parse, cheng2018cspn, Mal2018SparseToDense, qiu2019deeplidar, yang2019DDP, teixeira2020aerial_dc, wong2020dc_vio, li2019ManneqinChallenge, zhang2018depthcompletion}.

% In our work, which falls under (c), the sparse depth input to the neural network is computed by a real-time VI-SLAM system~\cite{KejianWuInverseFilter}.
% %
% With the aid of inertial measurement unit (IMU), we overcome the lack of metric scale as compared to approach (a).
% %
% Specifically, inspired by~\cite{qiu2019deeplidar}, we estimate a dense depth by fusing the RGB image, the surface normal, and the sparse depth of the environment.
% %
% While the surface normal is obtained via deep neural network from RGB image~\cite{Huang19FrameNet}, the sparse depth is obtained deterministically from the VI-SLAM. 
% %
% As recent studies~\cite{teixeira2020aerial_dc, wong2020dc_vio} show, there is a large performance degradation when inputting the sparse depth from VI-SLAM's point cloud to a pre-trained depth completion network.
% %
% This is due to 3 key differences between the 3D points triangulated by VI-SLAM and the point cloud directly measured from Kinect or LiDAR: Accuracy, density, and topology.
% %
% Specifically, the VI-SLAM point cloud comprises sparse points ($\simeq$ 0.5$\%$ of image’s pixels) that are tracked between images and triangulated via camera’s poses viewing these points. 
% %
% Hence there is a high variation in the accuracy of these points, depending on the quality of tracking and the pose estimation methods.
% %
% Last but not least, the sparse point cloud is resulted from pixels in images that are reliably tracked in multiple frames, they are usually located at high texture surfaces or at the joints of multiple surfaces due to their high variances of the surrounding pixels' photometrics~\cite{FREAK, ORB, SIFT, shi1994klt}. 
% %
% These differences constitute a domain gap between the training data (sparse point from LiDAR or random sample from Kinect) and the testing one (VI-SLAM point cloud). 
% %
% In addition to the characteristics of the point cloud, the camera up vector directions of the images taken in the large indoor datasets (ScanNet~\cite{Dai2017scannet}, NYUv2~\cite{Silberman:ECCV12}, Matterport3D~\cite{Matterport3D}) are biased to be aligned with gravity~\cite{saito2020roll_depth}. 
% %
% This results in, during inference time, an additional performance degradation to available pre-trained depth completion network~\cite{cheng2018cspn} and optical-flow to depth~\cite{liu2019neuralrgbd}. 
% %
% In this work, we tackle the domain gap caused by the point cloud input and the general viewing directions.

In our work, which falls under (c) and is inspired by~\cite{qiu2019deeplidar}, we seek to estimate dense depth by fusing RGB images, learned surface normals, and sparse depth information. 
%
In contrast to~\cite{qiu2019deeplidar} that uses LiDAR, we obtain the sparse points from a real-time visual-inertial SLAM (VI-SLAM) system~\cite{KejianWuInverseFilter}. 
%
There are thee key differences between the point clouds directly measured by a Kinect or a LiDAR and those estimated by VI-SLAM: Density, accuracy, and spatial distribution.
%
In particular, the VI-SLAM point cloud comprises sparse points ($\simeq$ 0.5\% of an image’s pixels) that are extracted and tracked across images and triangulated using the camera's estimated poses. 
%
For this reason, the accuracy of these points varies widely, depending on the local geometry and the camera's motion. 
%
Moreover, the VI-SLAM points are not uniformly distributed across an image.
%
They are usually found on high-texture surfaces, while textureless areas such as walls, floors, and ceilings that are ubiquitous in man-made environments often contain significantly fewer points. 
%
Due to this large domain gap, networks trained using Kinect or LiDAR data suffer from a significant performance degradation when
given 3D points triangulated by VI-SLAM as sparse depth information~\cite{teixeira2020aerial_dc, wong2020dc_vio}.
%
Furthermore, in large-scale indoor datasets (ScanNet~\cite{Dai2017scannet}, NYUv2~\cite{Silberman:ECCV12}, Matterport3D~\cite{Matterport3D}), the images are usually aligned with gravity~\cite{saito2020roll_depth}. 
%
During inference time, this bias results in further performance degradation of the depth completion networks~\cite{cheng2018cspn}, as well as optical-flow to depth networks trained on these data~\cite{liu2019neuralrgbd}. 
%
%In this work, we tackle the domain gap caused by the point cloud input and the general viewing directions.

A straightforward approach to address the domain gap and the lack of images from various vantage points is to collect and process more data and re-train the network. 
%
This, however, is both labor and time intensive. 
%
Alternatively, 3D mesh reconstructions from RGB-D sequences (e.g., BundleFusion~\cite{dai2017bundlefusion}, BAD-SLAM~\cite{schops2019badslam}, etc.) can be employed to synthesize novel views of RGB images. 
%
The accuracy of the 3D mesh, however, is usually not sufficient and the quality of the resulting data depends on many factors, e.g., the overlap between frames, the sparse points tracking error, etc. 
%
For this reason, in our work, we employ the VI-SLAM point cloud when training the depth estimation network while incorporating the VI-SLAM estimate of gravity direction to reduce the effect of ``unseen orientation."
%
Specifically, to address the domain gap issue in the point cloud, we first train a network using sparse depth input from the point cloud generated by VI-SLAM, instead of randomly sampling from the ground-truth depth (e.g., \cite{cheng2018cspn}). 
%
Furthermore, to increase the density of the point cloud, we leverage the planar structures commonly found indoors. 
%
Secondly, to solve the domain gap in viewing directions, we align each input image taken with ``unseen orientation" to a rectified orientation that the pre-trained network is more familiar with, using the gravity direction estimated from VI-SLAM.
%
We show that this approach not only improves the performance on images taken with familiar orientations, but also achieves satisfactory generalization on the unfamiliar ones.
% 
In summary, our main contributions are:
\begin{itemize}
    \item We introduce an efficient approach to improve the generalization of the VI-SLAM depth completion that leverages (i) the planar geometry of the scene and (ii) the camera's orientation with respect to gravity.
    \item We implement a full pipeline from VI-SLAM to dense depth estimation for evaluation on Azure Kinect~\cite{KinectAzure} and perform extensive experiments that demonstrate the advantages of our method over state-of-the-art approaches on dense-depth estimation~\cite{liu2019neuralrgbd, cheng2018cspn}.
\end{itemize}


==> iros_2020_arxiv/tex/02_related_work.tex <==
\section{Related Work}
\textbf{Single-view depth estimation}. Depth estimation from a single image has been studied by early works such as~\cite{saxena2006learning} which is based on handcrafted features.
%
More recently, numerous deep learning-based approaches have appeared (e.g., \cite{fu2018dorn,eigen2014depth,laina2016DeeperDepthPrediction, liu2015learning}) for estimating dense depth.
%
Note, however, that given a single image, the pixels' depths cannot be determined only from local features; hence data-driven approaches have to rely on the global context of the image, which is learned from the training data.
%
Therefore, despite the surprisingly good performance when trained and tested with images from the same dataset, they exhibit poor generalization on cross-dataset experiments~\cite{li2018megadepth}.

\textbf{Multi-view depth estimation}. One way to overcome the single-view depth estimation challenges is to consider multiple camera poses and optical flow.
%
Specifically, the scene depth can be recovered up to scale, given information from multiple views, or with metric scale if the poses are estimated with the aid of other sensors (e.g., IMU).
%
In particular, \cite{ummenhofer2017demon} takes two images as input, estimates the optical flow as an intermediate result, and refines the depths as well as the poses iteratively. 
%
On the other hand, \cite{zhou2018deeptam} computes the photometric errors by warping adjacent images to the current one, and inputs them along with the current image to neural network.
%
Lastly, \cite{liu2019neuralrgbd} estimates a probability distribution for the depth, instead of a single depth, and refines the initial depth estimates from a neural network by warping the depth distribution of adjacent images and fusing them in a Bayesian fashion.
%
These methods implicitly estimate depth from poses and optical flow using exclusively neural networks, instead of computing the depths of at least some points directly from geometry. As shown in~\cite{li2019ManneqinChallenge}, employing these sparse or semi-dense depths as the input of neural network results in higher performance as compared to relying on the optical flow.


\textbf{Depth completion from RGB and sparse depth}.
A key difference between the methods described hereafter and the previous two families of approaches is that the domains of their inputs are significantly different. 
%
Specifically, the RGB image has a well-defined range of values for all pixels, while the sparse depth image has only few valid values where the majority of the pixels' depths are unknown. 
%
To address this domain difference, many approaches such as \cite{eldesokey2019confidence, huang2019hms} propose normalized convolution and upsampling layers so that the missing pixels will not be processed in the convolution kernels.
%
% On the other hand, \cite{jaritz2018sparse, van2019sparse} show separate treatment of the sparse input channel might not be necessary and with proper training, applying the standard convolution operations can achieve superior results.
% 
On the other hand, methods such as \cite{jaritz2018sparse, van2019sparse,Mal2018SparseToDense, ma2019selfsupervised, lee2019depth} do not treat the sparse normal input differently, which indicates with proper training applying standard convolution can achieve comparable results.
% 
% % \cite{Mal2018SparseToDense} concatenates the color and sparse depth images to input to the network to predict the dense depth and augment the training by applying small roll rotations (5 deg) to achieve better generalization.
% % %
% % \cite{Mal2018SparseToDense}, however, employs different network structure based on the dataset used, and hence is not generalizable.
% % %

A different approach proposed by \cite{qiu2019deeplidar} showed that employing a network to compute the surface normals based on the RGB image and using the normals as an additional input to the later layers can improve the network's performance.
%
Moreover, it was proposed to concatenate color/normal channels and sum the depth channels for the skip-connections between the encoder and decoder.
%
As we show in our ablation study, while this design choice results in improvement on the same scenes, it reduces the generalizability to, e.g., data collected from different devices.
% % \cite{ma2019selfsupervised} extends \cite{Mal2018SparseToDense} by using an early fusion scheme instead of concatenation and employs a single network design for all datasets. 
% % %
% % They, however, employ P3P RANSAC followed by PnP to align monocular image sequences for their photometric term and hence do not generalize well to indoor scenes with many textureless regions where P3P and PnP might fail.
% % %
% % Yang~\etal~\cite{yang2019DDP} replace the smoothness loss in training with a learned posterior regularize depth prediction using a conditional prior network (CDN), which itself is trained in another dataset. 
% % %
% % This approach does not generalize, however, since the CDN needs to be re-trained to be applied to new scenes.
% % \cite{imran2019depth} addresses accurate depth estimation at object boundaries by introducing depth coefficients, a change of representation of depth from a real number to a linear combination discrete bins, and employs cross-entropy loss instead for training. %
% % On the other hand, \cite{lee2019depth} employs two networks, one to produce the intermediate dense depths, and the other to compute weights used in combination with the output of the first network to produce the final depth.
% % \cite{qiu2019deeplidar} showed that employing a network to compute the surface normal using the color image and using the normals as an additional input to the later layers can improve the performance of the network. In this work, it was proposed to concatenate color/normal channels and sum the depth channels for the skip-connections between the encoder and decoder. We will show in our ablation study that while this choice of design does result in improvement on the same scenes, it will reduce the generalizability to e.g., data collected from different devices.
% A different approach for depth completion was proposed by \cite{zhang2018depthcompletion}, where a network predicts the surface normal and occlusion boundaries from the color image, and the depth completion is as the solution to a sparse least-squares minimization problem.
% The minimization step, however, is time consuming and in this approach hallucination of depth for isolated parts of the scenes with no sparse depth measurements is impossible.
% Other works such as \cite{Mal2018SparseToDense, ma2019selfsupervised} employ depth and image concatenation or early fusion to infer depth of the scene, while \cite{lee2019depth, qiu2019deeplidar} employ a two-layer scheme where an intermediate representation of the input is first generated (different depth proposals, and surface normal estimates, respectively) and then processed to generate the final depth estimate.
%
% A different approach was proposed by \cite{zhang2018depthcompletion} where the surface normal and occlusion boundaries are employed to propagate the depth values through solving a least-squares minimization.
%
%

In~\cite{cheng2018cspn}, Cheng et al. introduced the convolutional spatial propagation network (CSPN), where the initial depth image and an affinity matrix are first produced by a CNN and then the depth is iteratively refined through a diffusion process involving the affinity matrix and the current depth estimate.
%
Furthermore, for the case of depth completion, CSPN employs validity masks to retain the depth of the sparse input, and hence does not allow the network to correct potentially noisy measurements.
%
As we will show in our experimental results, this policy will lead to loss in accuracy when the input depth is noisy.

Closely related to our work are those of \cite{teixeira2020aerial_dc} and \cite{wong2019voiced}.
%
In \cite{teixeira2020aerial_dc}, a system to compute dense depth from either LiDAR or SLAM point-cloud on-board MAVs is described using the confidence propagation network similar to \cite{eldesokey2019confidence}.
%
Since, however, their focus is on real-time performance on devices with limited resources, their accuracy is lower than the state of the art.
%
As in our work, \cite{wong2019voiced} also employs a VI-SLAM system to generate the sparse input. Moreover, it uses a two-step process to first extend the depth data from the sparse 3D point cloud and then combine them with the RGB image as the input to a network that produces the final dense-depth image.
%
In particular, \cite{wong2019voiced} first employs Delaunay triangulation~\cite{barber1996quickhull} to fit a triangular mesh on the sparse points of the image and then computes the depth of all the pixels falling within each triangle using its plane equation. 
%
Note that the accuracy of this approach depends heavily on the assumption that the triangles match with the planar surfaces of the image's scene, which, in general, is not true.\footnote{Another contribution of \cite{wong2019voiced} is creating visual-inertial datasets for depth estimation. However, it does not have ground-truth surface normal, which our networks relies on. Therefore, we instead employ Scannet~\cite{Dai2017scannet}, with surface normal readily available from 3D mesh, to train our network. As for evaluating generalization capability, we collected our own dataset with sufficient roll and pitch variation (which is not the case for the dataset of~\cite{wong2019voiced}) to highlight the effect of incorporating gravity.}



==> iros_2020_arxiv/tex/03_method.tex <==
\begin{figure*}[ht]
\includegraphics[width=\textwidth]{figs/overview_largepoints.pdf} 
\centering
\caption{Overview of the system. At each keyframe, the VI-SLAM (Sec.~\ref{ssec:slam}) processes images and IMU measurements to compute (i) the gravity direction which is provided to the surface-normal network (Sec.~\ref{ssec:normal}), and (ii) the sparse depth image. The sparse depth enrichment module (Sec.~\ref{ssec:partial_depth}) increases the density of the sparse-depth image using information about planes in the image. This is provided by the plane detection network (Sec.~\ref{ssec:mask}) that classifies image pixels as belonging to a particular plane and the surface normal network that estimates the normal of each pixel. The depth completion network (DCN) (Sec.~\ref{ssec:infer_depth}) employs the RGB image, the pixel normals, and the enriched sparse-depth image to produce a dense depth image.}
\label{fig:overview}
\end{figure*}

\section{Technical Approach}\label{sec:method}
In this paper, we propose a method to accurately predict dense depths using only sensors available on most mobile devices, i.e., a camera and an IMU.
%
Fig.~\ref{fig:overview} depicts an overview of our system, where the depth completion network (DCN) estimates the dense depth from the following inputs:
%
(i) the RGB image, (ii) a sparse depth image based on the 3D points triangulated by the VI-SLAM, and (iii) the
surface normal map predicted by another CNN. As shown experimentally by~\cite{qiu2019deeplidar} and evident in our ablation studies, (iii) improves the accuracy of depth estimation. 

%
Specifically, we employ VI-SLAM~\cite{KejianWuInverseFilter} (see Sec.~\ref{ssec:slam}), which takes as input images and IMU measurements, to compute the \emph{sparse 3D point cloud} observed by the camera.
%
Then, the \emph{sparse depth image} is obtained by projecting the point cloud to the camera frame.
%
Additionally, a CNN predicts the \emph{surface normal} of every pixel in the RGB image (see Sec.~\ref{ssec:normal}) while leveraging the gravity direction estimated by the VI-SLAM to improve its accuracy.
%
Note that although the sparse depth image from the VI-SLAM can be used directly as input to the DCN, we seek to first increase its density by performing a sparse-depth enrichment step.
%
To do so, we extract the \emph{planar patches} of the image using a CNN (see Sec.~\ref{ssec:mask}), and use the estimated normals along with any 3D points that fall inside a plane, to compute a denser depth representation of the scene (see Sec.~\ref{ssec:partial_depth}).
%
Finally, the DCN (see Sec.~\ref{ssec:infer_depth}) computes the dense depth estimate based on the RGB image, the enriched sparse depth image, and the surface normals.

\subsection{VI-SLAM: Sparse Depth Image Generation}\label{ssec:slam}
In this work, we employ the inverse square-root sliding window filter (SR-ISWF)~\cite{KejianWuInverseFilter} to estimate in real-time camera poses and 3D feature positions.
%
Specifically, at each time step the SR-ISWF extracts FAST~\cite{FAST} corners in the current image, and tracks them by matching their corresponding ORB descriptors~\cite{ORB} to the previous images.
%
The SR-ISWF then fuses the IMU measurements and the 2D-to-2D feature tracks across the sliding window to estimate the camera's motion along with the features' positions.

Every time the SR-ISWF processes an image, we project all visible 3D features on the image and use their depth (i.e., their Z component) to create the sparse depth image. The SR-ISWF also computes the gravity direction which is passed to the surface normal network.
%we generate a sparse depth image containing, at each pixel, the depth (i.e., the $Z$ component) of the visible features by projecting the currently visible point cloud onto the image frame along with the gravity direction\footnote{Note that the scale and the gravity direction are observable in a visual-inertial system~\cite{Hesch_TRO_14}.}.
%
%The gravity direction is passed to the surface normal network, and the resulting surface normal along with the sparse point cloud and plane mask is transmitted to the sparse depth enrichment module.
%
%The depth completion network then processes the surface normal, the color image, and the enriched depth to produce the dense depth.


\subsection{Surface Normal Network}\label{ssec:normal}

%
% \begin{figure}[h]
% \includegraphics[width=0.3\textwidth]{figs/error-distribution-crop.pdf} 
% \centering
% \caption{Error distribution of the surface normal over the camera frame reference (Y-axis corresponds to up vector direction of the image. The area around the Y-axis and the vector coplanar to XZ has smaller error than other part of the unit sphere, this suggests that the ScanNet training set has many images that their gravities align with the up vector of the camera.}
% \label{fig:angular_error_distribution}
% \end{figure}

\begin{figure}[ht]
\includegraphics[width=0.5\textwidth]{figs/sn_error_in_roll.pdf} 
\centering
\vspace{-5mm}
\caption{Top row: Input image from Azure Kinect along with the gravity aligned image; the performance of FrameNet is satisfactory. Bottom row: Input image with significant roll component, resulting in poor performance. Warping the input based on the gravity direction before passing it through the CNN improves the performance in both cases.}
\label{fig:surface_normal_error_with_roll}
\end{figure}

%
\begin{figure*}[ht]
\includegraphics[width=\textwidth]{figs/planes_annotation.pdf} 
\centering
\vspace{-7mm}
\caption{We refine the imprecise plane annotation: (a) Given an imprecise plane instance, (b) we fit a plane using the depth from ScanNet with a strict threshold, which produces a set of sparse, yet accurate, points. (c) Using the point set, we incrementally grow the planar region based on the surface normal from FrameNet. (d-e) This refinement allows us to precisely label the plane instances.}
\label{fig:annotation_cleanup}
\end{figure*}

As it will become evident from our experimental validation, the performance of the DCN depends on the accuracy of the surface normals prediction. In particular, training state-of-the-art surface-normal-estimation networks such as the FrameNet~\cite{Huang19FrameNet} on large-scale indoor datasets (e.g., ScanNet~\cite{Dai2017scannet}, NYUv2~\cite{Silberman:ECCV12}, Matterport3D~\cite{Matterport3D}) does not yield satisfactory results. 
%
This is due to the fact that the FrameNet's surface-normal estimator's performance degrades significantly when tested on images whose roll angles deviate substantially from the vertically-aligned images used during training (see Fig.~\ref{fig:surface_normal_error_with_roll}).
%
% More analysis on the performance degradation of ScanNet pretrained surface normal estimation network on gravity-nonaligned frames can be found in~\cite{Do2020SurfaceNormal}.

To address this issue, we follow the approach of~\cite{Do2020SurfaceNormal} to warp the input image so that the gravity, which is estimated from IMU, is aligned with the image's vertical axis.
%
Note that, in this paper, we are interested in how the accuracy of surface normal prediction affects the depth completion performance, rather than solely focusing on the surface normal performance as in~\cite{Do2020SurfaceNormal}.
% Note that in order to preserve the spatial information in the image, we do \textit{not} remove the \textit{pitch} component when the angle between the gravity direction and the vertical axis of the image is more than 30\degree. 
% This imposes a negative impact on the depth completion network that takes surface normal as the intermediate representation.
% Fig.~\ref{fig:angular_error_distribution} shows the surface normal prediction's error distribution over the ScanNet test dataset, we can see that the network performs well on the ground surface where the gravity is almost aligned with the up vector (green axis) of the image frame of reference, which constitute a large amount of ScanNet dataset (77\% of training images).
%
% To overcome the lack of training data in pitch and especially roll, in this work, we warp the input image such that (i) the roll component (image in-plane rotation) is removed and (ii) the gravity direction in the image's frame of reference is aligned with the image's up-vector when the angle between the gravity and the up-vector is less than 30 degree. 
% %
% The first condition is to remove the roll component of the image while the second one is to align the image with the orientation of the significant training scenes on ScanNet (see Fig~\ref{fig:surface_normal_error_with_roll}).
%

The idea of using gravity from VI-SLAM has been proposed in~\cite{fei2019geosupervised} as a regularization for a depth-prediction network during \textit{training} time.
%
In contrast, in our work we employ the online estimated gravity to improve the generalization during \textit{inference} time.
%
Recently, \cite{saito2020roll_depth} proposed to remove the roll angle from an image by using the orientation estimated from monocular SLAM~\cite{ORBSLAM}. This method, though, lacks global information hence it relies on the assumption that the first camera's view is aligned with gravity.
%
In contrast, and due to the observability of gravity in VI-SLAM system~\cite{Hesch_TRO_14}, our method makes no assumptions about the camera's motion.
% On the other hand, because the gravity estimated using VI-SLAM system is observable~\cite{Hesch_TRO_14}, our method is more robust in online applications.


\subsection{Plane Detection}\label{ssec:mask}
A key idea behind our approach is to take advantage of planar surfaces present in the scene to enrich the sparse depth image (see Sec.~\ref{ssec:partial_depth}).
%
To do so, we predict plane masks on the image using a CNN. 
%
Specifically, we leverage the ground-truth plane masks from Plane-RCNN~\cite{Liu2019planercnn} which employs the 3D mesh reconstruction created from ScanNet~\cite{Dai2017scannet} for the multi-plane instance proposals.
%
Unfortunately, the resulting plane annotations are misaligned as shown in Fig.~\ref{fig:annotation_cleanup}. 
%
Hence, to obtain reliable training data, Plane-RCNN proposed a heuristic method to detect this misalignment based on the discrepancies between the projected 3D mesh reconstruction on each image and their corresponding depth, and then drop any frames with large discrepancies during training.
%
While effective, this method discards a large set of planes annotations during training, which can potentially degrade the plane detector's performance.

To address this problem, we employ RANSAC-based~\cite{Fischler1981ransac} plane fitting and region growing to refine the plane annotations. 
%
Specifically, for each annotated plane from Plane-RCNN, we employ 3pt RANSAC, using the corresponding depth  from ScanNet and a strict inlier threshold (2 cm) to fit a plane.
%
This yields only a small set of inliers due to the imprecise depth measurements. 
%
Given the initial inliers, we grow the coplanar region through neighboring pixels based on two criteria: (i) the distance of each 3D point to the plane is less than 20 cm and (ii) the corresponding surface normal from FrameNet~\cite{Huang19FrameNet} is close (less than 30$^{\circ}$) to the plane's normal. 
%
If the plane computed through this process is substantially smaller than the annotation, we discard the annotation. 
%
By applying this method to all the annotated planes we are able to accurately compute the plane instances (see Fig.~\ref{fig:annotation_cleanup}) and ensure that the planes are well-aligned with the RGB images.
%
Lastly, we employ the improved annotations as ground-truth to train a Mask~R-CNN~\cite{he2017maskrcnn} network for plane detection.
% Our method is summarized in Algorithm~\ref{alg:plane_refining}.

% \begin{algorithm}[t]
%   \caption{Refinement of plane annotation}
%   \textbf{Input: } Plane instance mask from Plane-RCNN $\mathcal{M}_{\mathcal{I}}$, depth image from ScanNet $d_{\mathcal{I}}$, normal image from FrameNet $\mathbf{n}_{\mathcal{I}}$
%   \textbf{Output: } Refined masks $\widetilde{\mathcal{M}}_{\mathcal{I}}$
%   \begin{algorithmic}[1]
%     \State set $\widetilde{\mathcal{M}}_{\mathcal{I}} = \emptyset$
%     \For{$\mathcal{I}$ in $\mathcal{D}$}
%     	\For{plane instance mask $m$ in  $\mathcal{M}_{\mathcal{I}}$}
%       		\State $m_{\textsc{inlier}}$ = RANSAC plane fitting ($m$, $d_{\mathcal{I}}$)
%       		\State $\tilde{m}$ = region grow($m_{\textsc{inlier}}$, $\mathbf{n}_{\mathcal{I}}$)
%       		\If{ $ \frac{|\tilde{m}|}{m} > \delta$ }
%         			\State Add $\tilde{m}$ to $\widetilde{\mathcal{M}}_{\mathcal{I}}$
%       		\EndIf
%       \EndFor
% \EndFor
% \State \Return $\widetilde{\mathcal{M}}_{\mathcal{I}}$
%   \end{algorithmic}
%   \label{alg:plane_refining}
% \end{algorithm}


\subsection{Sparse Depth Enrichment}\label{ssec:partial_depth}

In this module, we enrich the sparse depth image by increasing the number of points it contains.
%
We focus on the parts of the scene where 3D point features project on a detected plane (see Sect.~\ref{ssec:mask}).
%
This process comprises the following two steps for estimating each plane's parameters:
% We first estimate the plane normal using the per-pixel normal estimates from the network (see Sect.~\ref{ssec:normal}) and then compute the plane distance.

\begin{enumerate}
    \item Plane Normal estimation: We randomly select a few pixels as plane-normal hypotheses and compare their directions to the rest of the plane's pixels to find the largest set of normal directions aligned within 10 degrees. We then assign as the plane's normal the average of the normal vectors of the largest set.
    \item Plane Distance estimation: Given the plane's normal $\mathbf{n}$, each 3D point $\mathbf{p}_i$ expressed in the camera's coordinate frame is a candidate for computing the plane's distance hypothesis $d_i = -\mathbf{n}^T\mathbf{p}_i$. As before, the one with the largest set of inliers is accepted, and the plane's distance $d$ is set to be the average distance of inliers.
\end{enumerate}
%
Next, we employ $\mathbf{n}$ and $d$ to compute the depth $z_i = -\frac{d}{\mathbf{n}^T \mathbf{b}_i}$ of each pixel, where $\mathbf{b}_i$ is its normalized homogeneous coordinate.
%
%
%
%We follow a similar approach with the depth of the points belonging on the plane.
%
% Since all plane parameters are now determined, we compute the depth of every pixel belonging to the plane (provided by the mask).
%
Hereafter, we refer to the depth image resulting from this process as the \textit{``incomplete depth image''} (see Fig.~\ref{fig:overview}).

Once the incomplete depth image is generated, we select only a subset of the points from it to form the enriched depth image provided to the DCN (see Fig.~\ref{fig:overview}).
%
The reason behind this choice is that often the 3D points triangulated by VI-SLAM may contain errors.
%
In this case, using the entire incomplete depth image as the input to the DCN will bias its output by implicitly forcing it to trust the depth values of many densely distributed pixels with erroneous estimates.
% This is due to the observation that the point cloud from the triangulated points of the VI-SLAM contains noise, hence using the entire incomplete depth as the input to the network will force it to process thousands of points with significant error, which significantly bias the output of the network.
%
On the other hand, our experiments (see Sect.~\ref{ssec:nyu}) and those of~\cite{teixeira2020aerial_dc} show that the DCN performs significantly better when the sparse depth image is uniformly distributed over the RGB image.
%
This requirement, however, is not typically satisfied by indoor areas containing large textureless surfaces.
%
Instead, 3D points often cluster in few parts of an image where high texture is observed.
%
% However, the distribution of the sparse points in indoor environments is typically not uniform and concentrate on well-textured areas.
%
By employing the proposed enrichment procedure, however, we are able to reduce the gap between the initial distribution of sparse depth and a uniform distribution.
%
As shown in Sect.~\ref{sec:exp_results}, sampling between 100-200 points from the incomplete depth image produces the best results.
%
% The reason as why employing more points can degrade the performance are (i) using more points skews the distribution of the sparse depth to that of the detected planes instead of the uniform distribution, and (ii) unlike when using the ground-truth depth to populate the sparse depth input, the incomplete depths contain noise due to incorrect plane mask an inexact surface normal and triangulated point depths and these errors can bias the network. 
% A plane can be uniquely determined by its normal and one 3D point, and hence we employ this geometric constraint to compute the depths using the sparse point cloud from Sec.~\ref{ssec:slam}, normals from Sec.~\ref{ssec:normal}, and plane masks from Sec.~\ref{ssec:mask}.

% We first refine the normal vectors on detected planes to determine the normal for each plane. To do so, for each plane detected in Sec.\ref{ssec:mask}, we apply Hough transform to the normals of all the pixels on the plane mask, to get a refined normal of the entire plane. Then, we replace the normals of all the pixels with the refined one. By doing so, we annotate each plane with one normal, as well as remove part of outliers from the imperfect prediction of the neural network in Sec.~\ref{ssec:normal}.

% Next, we generate depths for planes where at least one sparse point is tracked. We leverage the 3D point cloud projection from Sec.\ref{ssec:slam} and the plane masks to collect all the sparse points lying on each detected plane. For each plane, we generate plane equation ($\mathbf{n}^T\mathbf{p}+d=0$, where $d$ is the distance from the origin to the plane) hypothesis by each sparse point on it and its normal, and take the one with the maximum number of sparse-point inliers. Afterwards, the depths of all the pixels on this plane are readily computed using the plane equation.

% The union of the depths of the planes computed in this section and those of the sparse point cloud from Sec.~\ref{ssec:slam} is used as the input of depth completion neural network described in Sec.\ref{ssec:infer_depth}. Note that the number of points on the planes is significantly greater than that of the sparse point cloud, which can potentially reduce the difficulty of the depth completion.


\subsection{Depth Completion Network}\label{ssec:infer_depth}
\begin{figure}[t]
\includegraphics[width=0.5\textwidth]{figs/decoder.png} 
\centering
\caption{Decoder structure. Features at different scales of the RGB, normal, and depth images are concatenated together, passed through convolution and upsampling, and then summed. A final convolution and upsampling is applied to compute the dense depth image.}
\label{fig:deep_comp}
\end{figure}
Our DCN is inspired by the Panoptic FPN~\cite{kirillov2019panoptic}.
%
Specifically, each of the RGB, normal, and the sparse depth images are processed through separate encoders, which compute four feature tensors per input corresponding to different layers of the ResNet.
%, as seen in Fig.~\ref{fig:deep_encoder}.
%
Before being processed by the decoder, we concatenate the features of the RGB, normal, and sparse depth images at each scale and apply convolution and upsampling, resulting in four feature tensors of size $128\times 60 \times 80$.
%
These are then summed together and passed through a final convolution and upsampling layer resulting in the dense-depth image (see Fig.~\ref{fig:deep_comp}).
%

% \begin{figure}[t]
% \includegraphics[width=0.45\textwidth]{figs/encoder.pdf} 
% \centering
% \caption{Encoder structure. Our network contains an instance of this encoder for each input (RGB, normal, sparse depth). The input is of the size $320 \times 240$, and $k$ is the number of channels (one for depth, three for color and normal images) and the encoder computes four feature vectors ($F_1, F_2, F_3, F_4$) of decreasing spatial dimensions but increasing the number of channels.}
% \label{fig:deep_encoder}
% \end{figure}



==> iros_2020_arxiv/tex/04_exp_results.tex <==
\section{Experimental Results}\label{sec:exp_results}
In what follows, we experimentally verify the performance of our method, and compare it to state-of-the-art approaches.
%
Although our target application is for VI-SLAM systems, the lack of visual-inertial training data has led us to employ RGB-D datasets (i.e., ScanNet~\cite{Dai2017scannet} and NYUv2~\cite{Silberman:ECCV12}) to train our networks.
%
To assess the performance on visual-inertial data and verify the generalization capability of our approach, we have also collected data using Azure Kinect~\cite{KinectAzure}.
%
In terms of depth error metrics, we report root mean square error (RMSE) in meters, and $E(\hat{D}, \delta)$, which specifies the percentage of the estimated depths $\hat{D}$ for which $\max(\frac{\hat{D}}{D},\frac{D}{\hat{D}}) < \delta$, where $D$ is the ground-truth depth.
%
For surface normal error metrics, we report mean absolute of the error (MAD), median of absolute error (Median), and the percentage of pixels with angular error below a threshold $\xi$ with $\xi = $ 11.25\degree, 22.5\degree, 30.0\degree.
% the percentages of pixels with the ratio between the predicted depth and the ground-truth depth less than $\delta$. Specifically,
% \begin{align}
%     E(\hat{D}, \delta) = \frac{\left| \Big\{ \hat{D}_i | \max(\frac{\hat{D}_i}{D_i},\frac{D_i}{\hat{D}_i}) < \delta  \Big\} \right|}{| \{D_i\} | } \times 100
% \end{align}
% where $D_i$ is the ground-truth depth and $\hat{D}_i$ is the corresponding depth predicted by the network, $\boldsymbol{card}$ determines the cardinality of a set, and $\delta \in \{1.05, 1.10, 1.25, 1.25^2, 1.25^3\}$.
% $\max(\frac{D_{pred}}{D_{gt}},\frac{D_{gt}}{D_{pred}}) < \delta$, where $D_{pred}$ is the depth predicted by the network, $D_{gt}$ is the ground-truth depth, and  $\delta \in \{1.05, 1.10, 1.25, 1.25^2, 1.25^3\}$, respectively.

% \subsection{Datasets and Setup}
% We perform experiments on three datasets, two of which are used for training separately (i.e., ScanNet and NYUv2), and the one collected by Azure Kinect sensor to test the generalizability of the approach.
% %
% In this section, we first provide detailed description of our datasets followed by our experimental setup.

% \textbf{ScanNet~\cite{Dai2017scannet} dataset}: 


\textbf{Experiment Setup}: All the networks in this paper have been implemented in PyTorch~\cite{pytorch}, and the original authors' code and provided network weights have been used for comparisons against other methods.
%
To train the DCN, we employ $L_1$ loss and the Adam optimizer~\cite{kingma2015adam} with a learning rate of $10^{-4}$.
%
We train the model for 20 epochs and report the best epoch on the corresponding dataset's validation set.
%
The training was done on an NVIDIA Tesla V100 GPU with 32GB of memory with a batch size of 16.
%
% The inference time for the surface normal network, plane detection, incomplete depth generation, and depth completion networks are X1, X2, X3, and X4 milliseconds, respectively, and hence the proposed approach is amendable to online use-cases.
%
%We used the pre-trained ResNet weights provided by PyTorch to initialize the image encoder and employed~\cite{he2015deep_rectifiers} to initialize other layers.
% We employed~\cite{he2015deep_rectifiers} to initialize all the layers.
%
Since the aspect ratio of the Azure Kinect dataset images is significantly different than those of ScanNet and NYUv2, we first crop them and then resize to $320\times 240$.
% 
For the ScanNet and NYUv2 we only apply resizing.
%
Our neural network code is available at \url{https://github.com/MARSLab-UMN/vi_depth_completion} along with our datasets.


\subsection{Comparison on ScanNet Datasets}\label{ssec:exp_scannet}
We train and evaluate different configurations of our approach on the ScanNet indoor datasets and compare our performance with NeuralRGBD~\cite{liu2019neuralrgbd}.
%
Although ScanNet does not contain inertial data, we leverage other available annotations to estimate (i) the gravity direction, and (ii) a 3D point cloud, required for our training and testing.
%
Specifically, we obtain the gravity direction from the normal direction of pixels labeled as the ground (by FrameNet~\cite{Huang19FrameNet}).
%
To compute the 3D point cloud, we first extract FAST corners~\cite{FAST}, track them via KLT~\cite{Kanade1981}, and remove outliers by employing the 5pt-RANSAC~\cite{Nister04}.
%
The inlier tracks are then triangulated using the provided camera poses to generate the sparse 3D point cloud (on average, for each image we compute 58 sparse depth values from the point cloud which corresponds to $0.07\%$ of pixels).
%
Lastly, we generate plane masks for the entire dataset and compute the incomplete depth images through the process described in Sect.~\ref{ssec:partial_depth}.
%
%We train and test on subset of the dataset that have at least $6,000$ pixels ($8\%$ of $320\times 240$ image) of generated incomplete depth.
%
% Once the pre-processing step is completed, our network is trained on the standard training split, and the evaluation is performed on a subset of the test split containing 11,000.
%
%

% We compare our method against NeuralRGBD~\cite{liu2019neuralrgbd} using their provided weights for ScanNet dataset.
%
%
% In what follows, we first quantify the accuracy of the sparse depth input generated by the triangulation and the incomplete depth.
%
% Subsequently, we verify our claim that DCN using the enriched depth as its input results in higher generalization accuracy.
%
%To do so, we train and test three DCNs on different depth inputs: (i) sparse depth (SD), (ii) incomplete depth (ID), and (iii) enriched depth.
% To do so, we train and test two DCNs on different depth inputs: (i) sparse depth (SD), and (ii) incomplete depth (ID).
%
% For testing the enriched depth, we employ the trained SD network of (i) and augment the input depth with different densities as described in Sect.~\ref{ssec:partial_depth}.
%
% Table~\ref{tab:scannet} presents the error statistics of the aforementioned configurations of our approach, as well as the comparison with NeuralRGBD (using their pre-trained model) on the same set of images.
%
%All comparisons have been done on the same images to ensure fairness of the results.
%
In Table~\ref{tab:scannet}, we evaluate the accuracy of the reconstructed sparse and incomplete depth inputs as well as the final depth output using the following configurations: 
%
% The configurations shown in Table~\ref{tab:scannet} are:
\begin{itemize}
    \item \emph{Triangulation}: The sparse depth resulting from projecting the 3D point cloud on the image.
    \item \emph{Incomplete Depth}: The incomplete depth images generated through the process described in Sect.~\ref{ssec:partial_depth}.
    \item \emph{NeuralRGBD}~\cite{liu2019neuralrgbd}: State-of-the-art in depth estimation from a sequence of images.
    \item \emph{Ours-SD}: DCN results trained and tested using the sparse depth as input.
    \item \emph{Ours-ID}: DCN results trained and tested using the incomplete depth as input.
    \item \emph{Ours-Enriched 100, 200}: Using \emph{Ours-SD} trained network with selecting 100, or 200 additional points from the incomplete depth to generate the enriched depth (see Sect.~\ref{ssec:partial_depth} and Fig.~\ref{fig:overview}).
\end{itemize}
% In this table, we provide the statistics of both the input, and the outputs of the networks.
% %
% Specifically, ``Trignaulation" indicates the accuracy of the sparse depth before the enrichment, and ``ID" shows the accuracy of the generated incomplete depth.
% %
% ``Ours-ID" denotes the network trained by incomplete depth as the input, and "Ours-SD" is the network trained using the sparse depth input.
% %
% Furthermore, ``Ours-SD+100 ID", ``Ours-SD+200 ID", and ``Ours-SD+2000 ID" denote the network of ``Ours-SD", but we enrich the sparse depth by sampling 100, 200, or 2000 points from the incomplete depth, respectively, for inference (see Sec.~\ref{ssec:partial_depth}).
%

As evident from Table~\ref{tab:scannet}, the error $E(\hat{D}, \delta)$ of the triangulated points and incomplete depths show that the inputs are relatively accurate.
%The high RMSE, however, indicates that there exist at least a few high-error points present in the input.
%
Furthermore, using the enriched depth with 100 points as input has slightly higher accuracy in the stricter metrics ($\delta=1.05,1.10$). % while it is comparable to sparse depth input in other metrics.
%
On the other hand, a denser enriched depth image comprising 200 points decreases the accuracy for the reasons explained in Sect.~\ref{ssec:partial_depth}. 
%
Although the network trained and tested using incomplete depth performs slightly better than both sparse and enriched depths for the ScanNet dataset, its performance degrades drastically on cross-dataset (see Sect.~\ref{ssec:exp_azure}).
%
% This could be explained by the fact that including a few more points gives the network more information about the approximate depth values throughout the image.
%
% This can be very useful because we are using feature trackers to determine the depth and hence the in contrast to the approaches using more uniformly sampled depth (e.g., LiDAR), our sparse depth will not be uniformly sampled on the image and only areas with high texture will contain sparse depth information.
% %
% By including small amount of information about depth of the planar and potentially textureless parts of the scene, we enable the network to infer better depth estimates throughout the image.
% %
% On the other hand, using too many points will cause this network to perform worse because the SD network was not trained on denser depth inputs.
%
% Moreover, the network trained on the incomplete depth image (Ours-ID) also performs sub-par to the enriched depth (Ours-Enriched-200) as it is biased by potentially inaccurate depths.
%
% In our experiments, the inaccuracy of the incomplete depth is mostly due to the point cloud and the plane normal is usually accurate.
Finally, these results show that our approach outperforms NeuralRGBD on all metrics, especially the stricter ones. 
%

% These results indicate that our network can propagate the depth information better, as compared to the NeuralRGBD which receives five neighboring images and their relative poses, hence potentially processing more information as compared to ours.
\begin{table}[t]
\caption{Performance of depth completion on ScanNet test set}
\vspace{-5mm}
\label{tab:scannet}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|ccccc|}
\hline
 &                 &                   &                   &   $E(\hat{D}, \delta)$       &                     &  \\ \cline{3-7}
 &	RMSE $\downarrow$ & 1.05 $\uparrow$ &	1.10$\uparrow$  &	1.25$\uparrow$ &	$1.25^2 \uparrow$ &	$1.25^3 \uparrow$ \\
\hline
\hline
Triangulation            & 0.153 & 75.89 & 92.19 & 98.51 & 99.64 & 99.89 \\
Incomplete Depth               & 0.201 & 66.39 & 85.30 & 96.64 & 99.05 & 99.60 \\
\hline
NeuralRGBD~\cite{liu2019neuralrgbd}          &	0.294         &	46.35          &	72.99          &	93.00         &	98.30 &	99.43 \\

Ours-SD &	0.266 &	54.09 &	78.41 &	94.68 &	\textbf{98.91} &	\textbf{99.71} \\
Ours-ID & \textbf{0.265} &	54.65       &	   \textbf{78.71}       & \textbf{94.72}	 & 98.85	 &	99.67 \\
Ours-Enriched 100 &  0.271 & \textbf{54.85} & 78.54 & 94.55 & 98.76 & 99.66  \\
Ours-Enriched 200  & 0.271 &	54.37 &	78.11 &	94.46 &	98.73 &	99.63 \\
\hline
\end{tabular}
}
\end{center}
\vspace{-5mm}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Comparison on NYUv2 Depth Dataset}\label{ssec:nyu}
To compare against the CSPN~\cite{cheng2018cspn}, we also test our approach on the NYUv2 datasets, comprised of color and depth images from 464 different indoor scenes acquired by a Microsoft Kinect sensor.
%
In our evaluation, we used the official 249 training scenes and sub-sampled $25,000$ color-depth image pairs for the network to train, while tested on the standard 654-image test set.
%
%Firstly, we pre-process NYUv2 by associating the color and depth images close in time, and project the depth to color image frames.
%
%Then, we sub-sample $25,000$ color-depth image pairs for the network to train.
% %
% Because the color and depth cameras operate at different variable frequencies, we associate each color image with the depth image close in time.
% %
% We then remove the pairs that have time difference more than 20 msec, or map multiple color images to a single depth image.
% %
% The remaining pairs are then sub-sampled to $25,000$ color-depth image pairs used for training.
% %
% The provided camera intrinsic and extrinsic parameters are then used to project the depth image to the color image's frame.
%
%Finally, we test on the standard 654-image NYUv2 test set.
%
Since NYUv2 does not provide camera poses, to generate the sparse depth, we first extract 2D-to-2D correspondences (see Sect.~\ref{ssec:exp_scannet}), and then sample from the ground-truth depth instead of projecting a 3D point-cloud as input to the DCN.
% Note that in contrast to the ScanNet, the NYUv2 dataset does not provide camera poses which prevents us from triangulating features.
%
% To circumvent this issue, we employ the same FAST-KLT pipeline used in ScanNet, but instead of using the triangulated features' depth we employ the ground-truth depth values.
%
% Furthermore, for the surface normal network, we employ the one trained on the ScanNet instead of re-training it on NYUv2, due to the unavailability of NYUv2's 3D surface reconstruction.
%
% Additionally, since we have already shown the superiority of the network trained by sparse depth (see Table~\ref{tab:scannet}), we do not train a network with depth incomplete input (Ours-ID) on this dataset.
%

Table~\ref{tab:nyu} shows the performance of the proposed approach compared to CSPN using their pre-trained model.
%
Note that the CSPN model has been trained on sparse depth generated by randomly sampling from the ground-truth depth.
%
In our tests, we compare the computed depth when the sparse depth is from 2D-to-2D tracks (denoted as ``Feature'' in Table~\ref{tab:nyu}), and by randomly sampling 200 points from the ground-truth (``Uniform'').
% We then train the DCN and compare to CSPN under two different conditions of the depth input: (i) Using the tracked feature locations to sample the input, and (ii) randomly sampling 200 points from the ground-truth.
%
% We evaluate the results by providing the sparse depth image using different sampling methods: (i)~Tracked features and their corresponding ground-truth depth values denoted by ``KLT" in Table~\ref{tab:nyu}, (ii)~Randomly sampled 200 points.
%
These results show that our approach outperforms CSPN in all metrics.
%
Additionally, the gap in performance when employing features is much larger than using random samples.
%
This is due to the distribution of FAST corners on the images, where more points are located on the textured areas as compared to the textureless ones.
%
% On the other hand, when using 200 random samples we receive depth information on the image uniformly.
% %
% Since CSPN is trained on uniform depth samples, it suffers from higher errors when the sparse depth input distribution is non-uniform, while ours performs well on both inputs.

%Note that since the depth input to the network for this dataset is the ground-truth, inclusion of any noisy depth value will degrade the performance of the network.
%
%Hence we do not consider sampling from the incomplete depth, which is contaminated by the noise of the surface normal estimation, for this dataset.
%
\begin{table}[t]
\caption{Performance of depth completion on NYUv2 test set}
\vspace{-5mm}
\label{tab:nyu}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|ccccc|}
\hline
 &                 &                   &                   &   $E(\hat{D}, \delta)$       &                     &  \\ \cline{3-7}
 &	RMSE $\downarrow$ &	1.05 $\uparrow$ &	1.10$\uparrow$  &	1.25$\uparrow$ &	$1.25^2 \uparrow$ &	$1.25^3 \uparrow$ \\
\hline
\hline
CSPN\cite{cheng2018cspn} (Feature)   & 0.46  & 69.31 & 78.39 & 86.47 & 91.65 & 94.57 \\
Ours-SD (Feature) & \textbf{0.20}  & \textbf{80.38} & \textbf{91.27} & \textbf{97.53} & \textbf{99.50} & \textbf{99.89} \\
\hline
CSPN\cite{cheng2018cspn} (Uniform)   & \textbf{0.18} & 87.56 & 94.17 & 98.24 & 99.59 & 99.88 \\
Ours-SD (Uniform) & \textbf{0.18} & \textbf{88.86} & \textbf{94.82} & \textbf{98.46} & \textbf{99.66} & \textbf{99.91}  \\
\hline
\end{tabular}
}
\end{center}
\vspace{-5mm}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Generalization Capability on Azure Kinect Datasets}\label{ssec:exp_azure}
In order to evaluate our DCN on datasets with visual-inertial data, and to better compare the generalization capability of our approach against the alternative ones, we collected 24 datasets in indoor areas using the Azure Kinect~\cite{KinectAzure}. 
%
Each dataset comprises color and depth images at 30~Hz, as well as IMU measurements at 1.6~KHz. 
%
The depth images are employed as the ground-truth, while the color images and the IMU measurements are processed by the VI-SLAM to compute the camera's poses and the triangulated feature positions.
%
These datasets produce a total of $\sim$8K keyframes which we use for evaluation.
%
Unless otherwise specified, all networks considered in this section are trained only on ScanNet dataset.

%
First, we present the performance and the effectiveness of our gravity alignment for the surface normal estimation (Sec.~\ref{ssec:normal}) on Azure Kinect datasets. 
%
% FrameNet~\cite{Huang19FrameNet} achieves state-of-the-art surface normal estimation by using DORN~\cite{fu2018dorn}, a high capacity network architecture which employs effective use of ASPP modules \cite{chen2017deeplab}\cite{Chen2017RethinkingAC} and maintains large spatial resolution in deep layers. 
%
Table~\ref{tab:surface_normal_azure} compares the proposed gravity alignment (see Sect.~\ref{ssec:normal}) against the following alternatives: (i) Vanilla - training with standard ground-truth surface normal and (ii) Warping augmentation - improving generalization by warping the input image with random rotation during training; on two categories of images (1) gravity aligned and (2) gravity non-aligned.
%
The network used in all cases is DORN~\cite{fu2018dorn}, and is trained with the truncated angular loss~\cite{Do2020SurfaceNormal}.
%
In these tests, we achieve satisfactory performance when evaluating DORN on the scenes with gravity aligned images (see Table~\ref{tab:surface_normal_azure}, Gravity-aligned frames).
%
Its performance, however, reduces drastically when the images have large pitch/roll rotations (see Table~\ref{tab:surface_normal_azure}, Gravity-nonaligned frames).
%
We attribute this degradation to the lack of training images with large pitch/roll angles. 
%
To assess the accuracy of our approach, we also compare against a naive data augmentation scheme that randomly warps each input image to provide the network with more diverse viewing-directions.
%which significantly improves the performance of the network especially on the gravity non-aligned frames as shown in Table~\ref{tab:surface_normal_azure}. 
%
% Furthermore, because a significant number of training scenes on ScanNet contain a lot of surface normal pointing in the gravity direction (e.g. floor), 
%
\begin{figure*}[h]
\includegraphics[width=\textwidth]{figs/qualitative_fig.pdf} 
\centering
\vspace{-8mm}
\caption{Qualitative results on gravity-nonaligned scenes.}
\label{fig:qualitative}
\end{figure*}
%
Finally, Table~\ref{tab:surface_normal_azure} shows that by warping in a direction aligned with the gravity obtained from VI-SLAM, our method outperforms both the baseline DORN and training with data augmentation (i.e., randomly warping images) in terms of generalization performance without requiring data augmentation, hence resulting in shorter training time.
%
\begin{table}[ht]
\caption{Performance of surface normal estimation on Azure Kinect dataset}
\vspace{-5mm}
\label{tab:surface_normal_azure}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|cccccc|}
\hline
% & & & & & & \\
Gravity-aligned frames & MAD$\downarrow$   & Median$\downarrow$ & RMSE$\downarrow$ & 11.25\degree$\uparrow$ & 22.5\degree$\uparrow$ & 30.0\degree$\uparrow$ \\
\hline
Vanilla                         & 9.15  & 4.89   & 15.91 & 80.83    & 90.83   & 93.41 \\
Warping Augmentation    & 9.31  & 4.61   & 17.23 & 81.88    & 90.59   & 92.95   \\
Gravity Alignment & \textbf{8.62}  & \textbf{4.26}   & \textbf{15.57} & \textbf{82.03}    & \textbf{91.17}   & \textbf{93.68}   \\
\hline
\hline
Gravity-nonaligned frames & MAD$\downarrow$   & Median$\downarrow$ & RMSE$\downarrow$ & 11.25\degree$\uparrow$ & 22.5\degree$\uparrow$ & 30.0\degree$\uparrow$ \\
\hline
Vanilla                         & 14.40 & 6.86   & 23.32 & 65.55    & 81.56   & 85.77   \\
Warping Augmentation     & 11.87 & 5.63   & 20.87 & \textbf{74.91}    & \textbf{86.48}   & 89.67   \\
Gravity Alignment  & \textbf{11.46} & \textbf{5.22}   & \textbf{19.88} & 74.24    & 86.29   & \textbf{89.75} \\
\hline
\hline
All frames & MAD$\downarrow$   & Median$\downarrow$ & RMSE$\downarrow$ & 11.25\degree$\uparrow$ & 22.5\degree$\uparrow$ & 30.0\degree$\uparrow$ \\
\hline
Vanilla                         & 11.37 & 5.41   & 19.31 & 74.35    & 86.48   & 89.95   \\
Warping Augmentation     & 10.62 & 5.09   & 19.19 & 78.31    & 88.48   & 91.27   \\
Gravity Alignment  & \textbf{10.03} & \textbf{4.65}   & \textbf{17.84} & \textbf{78.33}    & \textbf{88.73}   & \textbf{91.74} \\
\hline
\end{tabular}}
\end{center}
\vspace{-5mm}
\end{table}

\begin{table}[ht]
\caption{Performance of depth completion on Azure Kinect dataset}
\vspace{-5mm}
\label{tab:azure}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|ccccc|}
\hline
 &                 &                   &                   &   $E(\hat{D}, \delta)$       &                     &  \\ \cline{3-7}
 &	RMSE $\downarrow$ &	1.05 $\uparrow$ &	1.10$\uparrow$  &	1.25$\uparrow$ &	$1.25^2 \uparrow$ &	$1.25^3 \uparrow$ \\
\hline
\hline
	
CSPN-NOISY       & 1.461  & 5.10  &  9.03 & 17.02 & 29.52 & 43.25 \\
CSPN-GT          & 1.465  & 8.10  & 11.20 & 17.93 & 29.49 & 42.69 \\
Ours-SD${}^{\dagger}$  & 0.913 & 11.70 & 22.55 & 47.96 & 74.85 & 88.03 \\
Ours-Enriched 100${}^{\dagger}$ & \textbf{0.814} & \textbf{15.09} & \textbf{28.74} & \textbf{57.93} & \textbf{82.23} & \textbf{91.48} \\
\hline
NeuralRGBD       & 0.717  & 20.03 &	36.25 &	65.25 &	86.28 &	94.59 \\
Ours-ID          & 0.534 &	18.64 &	35.54 &	71.00 &	93.84 &	98.20 \\
Ours-SD          & 0.524 &  19.96 & 37.55 & 73.78 & 94.24 & 98.52 \\
Ours-Enriched 100   & 0.496 &  24.21 & \textbf{44.34} & 79.07 & 95.32 & 98.71 \\
% Ours-SD+200 ID   & 0.496 &	24.07 &	44.20 &	78.96 &	95.27 &	98.69  \\
Ours-Enriched 100+g & \textbf{0.490} &  \textbf{24.26} & 44.31 & \textbf{79.23} & \textbf{95.65} & \textbf{98.95} \\
% Ours-SD+200 ID+g & \textbf{0.489} &	24.09 & 44.19 & 79.17 & 95.61 & 98.93 \\
\hline
\end{tabular}
}
\end{center}
\vspace{-5mm}
\end{table}

Table~\ref{tab:azure} presents the depth completion performance of our method, as compared to the NeuralRGBD and CSPN, on the Azure Kinect dataset.
%
To properly compare with the pretrained NeuralRGBD and CSPN, we separately train our DCN network on ScanNet and NYUv2 (denoted with~${}^{\dagger}$).
% Both our network and NeuralRGBD are trained on ScanNet, while CSPN is trained on NYUv2.
%
Since CSPN is trained using points sampled from the ground-truth depth, besides evaluating its performance on the triangulated point cloud (CSPN-NOISY), we also assess its performance when the sparse depth of the same locations is extracted from the ground-truth depth (CSPN-GT).
%
In addition to the previous results, we also include our depth enrichment method with the surface normal computed using our proposed gravity-aware network (Ours-Enriched 100+g).
%
Table~\ref{tab:azure} shows that our algorithm significantly outperforms the alternative methods in all metrics for cross-dataset evaluation, thus confirming the generalization capability of depth enrichment approach for the network trained on either NYUv2 or ScanNet.
%
In addition, it shows that the impact of the depth enrichment method is more significant than the accuracy of the surface normal prediction.
%
Fig.~\ref{fig:qualitative} qualitatively illustrates our method for  gravity-nonaligned images.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\subsection{Comparison on NYUv2 Depth Dataset}\label{ssec:nyu}
To compare against the CSPN~\cite{cheng2018cspn}, we also test our approach on the NYUv2 datasets, comprised of color and depth images from 464 different indoor scenes acquired by a Microsoft Kinect sensor.
%
In our evaluation, we used the official 249 training scenes and sub-sampled $25,000$ color-depth image pairs for the network to train, while tested on the standard 654-image test set.
%
%Firstly, we pre-process NYUv2 by associating the color and depth images close in time, and project the depth to color image frames.
%
%Then, we sub-sample $25,000$ color-depth image pairs for the network to train.
% %
% Because the color and depth cameras operate at different variable frequencies, we associate each color image with the depth image close in time.
% %
% We then remove the pairs that have time difference more than 20 msec, or map multiple color images to a single depth image.
% %
% The remaining pairs are then sub-sampled to $25,000$ color-depth image pairs used for training.
% %
% The provided camera intrinsic and extrinsic parameters are then used to project the depth image to the color image's frame.
%
%Finally, we test on the standard 654-image NYUv2 test set.
%
Since NYUv2 does not provide camera poses, to generate the sparse depth, we first extract 2D-to-2D correspondences (see Sect.~\ref{ssec:exp_scannet}), and then sample from the ground-truth depth instead of projecting a 3D point-cloud as input to the DCN.
% Note that in contrast to the ScanNet, the NYUv2 dataset does not provide camera poses which prevents us from triangulating features.
%
% To circumvent this issue, we employ the same FAST-KLT pipeline used in ScanNet, but instead of using the triangulated features' depth we employ the ground-truth depth values.
%
% Furthermore, for the surface normal network, we employ the one trained on the ScanNet instead of re-training it on NYUv2, due to the unavailability of NYUv2's 3D surface reconstruction.
%
% Additionally, since we have already shown the superiority of the network trained by sparse depth (see Table~\ref{tab:scannet}), we do not train a network with depth incomplete input (Ours-ID) on this dataset.
%

Table~\ref{tab:nyu} shows the performance of the proposed approach compared to CSPN using their pre-trained model.
%
Note that the CSPN model has been trained on sparse depth generated by randomly sampling from the ground-truth depth.
%
In our tests, we compare the computed depth when the sparse depth is from 2D-to-2D tracks (denoted as ``Feature'' in Table~\ref{tab:nyu}), and by randomly sampling 200 points from the ground-truth (``Uniform'').
% We then train the DCN and compare to CSPN under two different conditions of the depth input: (i) Using the tracked feature locations to sample the input, and (ii) randomly sampling 200 points from the ground-truth.
%
% We evaluate the results by providing the sparse depth image using different sampling methods: (i)~Tracked features and their corresponding ground-truth depth values denoted by ``KLT" in Table~\ref{tab:nyu}, (ii)~Randomly sampled 200 points.
%
These results show that our approach outperforms CSPN in all metrics.
%
Additionally, the gap in performance when employing features is much larger than using random samples.
%
This is due to the distribution of the FAST corners on the image, where more points are located on the textured areas as compared to the textureless ones.
%
% On the other hand, when using 200 random samples we receive depth information on the image uniformly.
% %
% Since CSPN is trained on uniform depth samples, it suffers from higher errors when the sparse depth input distribution is non-uniform, while ours performs well on both inputs.

%Note that since the depth input to the network for this dataset is the ground-truth, inclusion of any noisy depth value will degrade the performance of the network.
%
%Hence we do not consider sampling from the incomplete depth, which is contaminated by the noise of the surface normal estimation, for this dataset.
%
\begin{table}[t]
\caption{Performance of depth completion on NYUv2 test set}
\vspace{-5mm}
\label{tab:nyu}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|ccccc|}
\hline
 &                 &                   &                   &   $E(\hat{D}, \delta)$       &                     &  \\ \cline{3-7}
 &	RMSE $\downarrow$ &	1.05 $\uparrow$ &	1.10$\uparrow$  &	1.25$\uparrow$ &	$1.25^2 \uparrow$ &	$1.25^3 \uparrow$ \\
\hline
\hline
CSPN\cite{cheng2018cspn} (Feature)   & 0.46  & 69.31 & 78.39 & 86.47 & 91.65 & 94.57 \\
Ours-SD (Feature) & \textbf{0.20}  & \textbf{80.38} & \textbf{91.27} & \textbf{97.53} & \textbf{99.50} & \textbf{99.89} \\
\hline
CSPN\cite{cheng2018cspn} (Uniform)   & \textbf{0.18} & 87.56 & 94.17 & 98.24 & 99.59 & 99.88 \\
Ours-SD (Uniform) & \textbf{0.18} & \textbf{88.86} & \textbf{94.82} & \textbf{98.46} & \textbf{99.66} & \textbf{99.91}  \\
\hline
\end{tabular}
}
\end{center}
\vspace{-5mm}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Generalization Capability on Azure Kinect Datasets}\label{ssec:exp_azure}
In order to evaluate our DCN on datasets with visual-inertial data, and to better compare the generalization capability of our approach against the alternative ones, we collected 24 datasets in indoor environments using the Azure Kinect~\cite{KinectAzure}. 
%
Each dataset comprises color and depth images at 30~Hz, as well as IMU measurements at 1.6~KHz. 
%
The depth images are employed as the ground-truth, while the color images and the IMU measurements are processed by the VI-SLAM to compute the camera's poses and the triangulated feature positions.
%
These datasets produce a total of $\sim$8K keyframes which we use for evaluation.
%
Unless otherwise specified, all networks considered in this section are trained only on ScanNet dataset.

%
First, we present the performance and the effectiveness of our gravity alignment for the surface normal estimation (Sec.~\ref{ssec:normal}) on Azure Kinect datasets. 
%
% FrameNet~\cite{Huang19FrameNet} achieves state-of-the-art surface normal estimation by using DORN~\cite{fu2018dorn}, a high capacity network architecture which employs effective use of ASPP modules \cite{chen2017deeplab}\cite{Chen2017RethinkingAC} and maintains large spatial resolution in deep layers. 
%
Table~\ref{tab:surface_normal_azure} compares the proposed gravity alignment (see Sect.~\ref{ssec:normal}) against the following alternatives: (i) Vanilla - training with standard ground-truth surface normal and (ii) Warping augmentation - improving generalization by warping the input image with random rotation during training; on two categories of images (1) gravity aligned and (2) gravity non-aligned.
%
The network used in all cases is DORN~\cite{fu2018dorn}, i.e., the proposed network architecture in FrameNet~\cite{Huang19FrameNet}.\footnote{In contrast to FrameNet that estimates a full frame of reference, we only use the surface normal component (the Z-axis of the frame) in our training.}
%
In these tests, we achieve satisfactory performance when evaluating DORN on the scenes with gravity aligned images (see Table~\ref{tab:surface_normal_azure}, Gravity-aligned frames).
%
Its performance, however, reduces drastically when the images have large pitch/roll rotations (see Table~\ref{tab:surface_normal_azure}, Gravity-nonaligned frames).
%
We attribute this degradation to the lack of training images with large pitch/roll angles. 
%
To assess the accuracy of our approach, we also compare against a naive data augmentation scheme that randomly warps each input image to provide the network with more diverse viewing-directions.
%which significantly improves the performance of the network especially on the gravity non-aligned frames as shown in Table~\ref{tab:surface_normal_azure}. 
%
% Furthermore, because a significant number of training scenes on ScanNet contain a lot of surface normal pointing in the gravity direction (e.g. floor), 
%
\begin{figure*}[h]
\includegraphics[width=0.95\textwidth]{figs/qualitative_cropped.pdf} 
\centering
\vspace{-3mm}
\caption{Qualitative results on gravity-nonaligned scenes.}
\label{fig:qualitative}
\end{figure*}
%
Finally, Table~\ref{tab:surface_normal_azure} shows that by warping in a direction aligned with the gravity obtained from VI-SLAM, our method outperforms both the network trained with data augmentation (i.e., randomly warping images) and current state-of-the-art method FrameNet~\cite{Huang19FrameNet} in terms of generalization performance without requiring data augmentation, hence resulting in shorter training time.
%
\begin{table}[ht]
\caption{Performance of surface normal estimation on Azure Kinect dataset}
\vspace{-5mm}
\label{tab:surface_normal_azure}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|cccccc|}
\hline
% & & & & & & \\
Gravity-aligned frames & MAD$\downarrow$   & Median$\downarrow$ & RMSE$\downarrow$ & 11.25\degree$\uparrow$ & 22.5\degree$\uparrow$ & 30.0\degree$\uparrow$ \\
\hline
Vanilla                         & 9.15  & 4.89   & 15.91 & 80.83    & 90.83   & 93.41 \\
Warping Augmentation    & 9.31  & 4.61   & 17.23 & 81.88    & 90.59   & 92.95   \\
Gravity Alignment & \textbf{8.62}  & \textbf{4.26}   & \textbf{15.57} & \textbf{82.03}    & \textbf{91.17}   & \textbf{93.68}   \\
\hline
\hline
Gravity-nonaligned frames & MAD$\downarrow$   & Median$\downarrow$ & RMSE$\downarrow$ & 11.25\degree$\uparrow$ & 22.5\degree$\uparrow$ & 30.0\degree$\uparrow$ \\
\hline
Vanilla                         & 14.40 & 6.86   & 23.32 & 65.55    & 81.56   & 85.77   \\
Warping Augmentation     & 11.87 & 5.63   & 20.87 & \textbf{74.91}    & \textbf{86.48}   & 89.67   \\
Gravity Alignment  & \textbf{11.46} & \textbf{5.22}   & \textbf{19.88} & 74.24    & 86.29   & \textbf{89.75} \\
\hline
\hline
All frames & MAD$\downarrow$   & Median$\downarrow$ & RMSE$\downarrow$ & 11.25\degree$\uparrow$ & 22.5\degree$\uparrow$ & 30.0\degree$\uparrow$ \\
\hline
Vanilla                         & 11.37 & 5.41   & 19.31 & 74.35    & 86.48   & 89.95   \\
Warping Augmentation     & 10.62 & 5.09   & 19.19 & 78.31    & 88.48   & 91.27   \\
Gravity Alignment  & \textbf{10.03} & \textbf{4.65}   & \textbf{17.84} & \textbf{78.33}    & \textbf{88.73}   & \textbf{91.74} \\
\hline
\end{tabular}}
\end{center}
\vspace{-5mm}
\end{table}
\begin{table}[ht]
\caption{Performance of depth completion on Azure Kinect dataset}
\vspace{-5mm}
\label{tab:azure}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|ccccc|}
\hline
 &                 &                   &                   &   $E(\hat{D}, \delta)$       &                     &  \\ \cline{3-7}
 &	RMSE $\downarrow$ &	1.05 $\uparrow$ &	1.10$\uparrow$  &	1.25$\uparrow$ &	$1.25^2 \uparrow$ &	$1.25^3 \uparrow$ \\
\hline
	
CSPN-NOISY       & 1.461  & 5.10  &  9.03 & 17.02 & 29.52 & 43.25 \\
CSPN-GT          & 1.465  & 8.10  & 11.20 & 17.93 & 29.49 & 42.69 \\
NeuralRGBD       & 0.717  & 20.03 &	36.25 &	65.25 &	86.28 &	94.59 \\
Ours-ID          & 0.534 &	18.64 &	35.54 &	71.00 &	93.84 &	98.20 \\
Ours-SD          & 0.524 &  19.96 & 37.55 & 73.78 & 94.24 & 98.52 \\
% Ours-SD+100 ID   & 0.496 &  24.21 & \textbf{44.34} & 79.07 & 95.32 & 98.71 \\
% Ours-SD+200 ID   & 0.496 &	24.07 &	44.20 &	78.96 &	95.27 &	98.69  \\
Ours-SD+100 ID+g & \textbf{0.490} &  \textbf{24.26} & \textbf{44.31} & \textbf{79.23} & \textbf{95.65} & \textbf{98.95} \\
% Ours-SD+200 ID+g & \textbf{0.489} &	24.09 & 44.19 & 79.17 & 95.61 & 98.93 \\
\hline
\end{tabular}
}
\end{center}
\vspace{-5mm}
\end{table}

Table~\ref{tab:azure} presents the depth completion performance of our method, as compared to the NeuralRGBD and CSPN, on the Azure Kinect dataset.
%
Both our network and NeuralRGBD are trained on ScanNet, while CSPN is trained on NYUv2.
%
Since CSPN is trained using points sampled from the ground-truth depth, besides evaluating its performance on the triangulated point cloud (CSPN-NOISY), we also assess its performance when the sparse depth of the same locations is extracted from the ground-truth depth (CSPN-GT).
%
In addition to the previous results, we also include our depth enrichment method with the surface normal computed using our proposed gravity-aware network (Ours-SD+100 ID+g).
%
Table~\ref{tab:azure} shows that our algorithms significantly outperforms the alternative methods in all metrics for cross-dataset evaluation, thus confirming the generalization capability of our approach.
%
Fig.~\ref{fig:qualitative} qualitatively illustrates our method for  gravity-nonaligned images.
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Ablation Studies}
In this section, we study the effect of different inputs on the performance of the network. Our main findings are: 

\noindent \textbf{Surface normal input improves the depth prediction}. Table~\ref{tab:inputs} verifies the effectiveness of the surface normal image as an additional input to the DCN, where we trained and tested a network using only the RGB and sparse depth images on the ScanNet dataset.
%
This is also in line with the findings of~\cite{qiu2019deeplidar}.
\begin{table}[ht]
\caption{Effect of the surface normal input (ScanNet)} %\hspace{\textwidth}
%Bottom: Better normal results in better depth (Gravity-nonaligned Azure)}
\vspace{-7mm}
\label{tab:inputs}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|ccccc|}
\hline
 &                 &                   &                   &  $E(\hat{D}, \delta)$      &                     &  \\ \cline{3-7}
 &	RMSE $\downarrow$ & 1.05 $\uparrow$ &	1.10$\uparrow$  &	1.25$\uparrow$ &	$1.25^2 \uparrow$ &	$1.25^3 \uparrow$ \\
\hline
\hline
w/o Normal &	0.342 &	45.65 &	69.38 &	90.14 &	97.57 &	99.38 \\
w/ Normal &	\textbf{0.266} & \textbf{54.09} & \textbf{78.41} & \textbf{94.68} & \textbf{98.91} &	\textbf{99.71} \\
\hline
% Ours-SD   &	0.540 & 15.58 & 31.33 & 70.81 & 93.86 & 98.11 \\
% Ours-SD+g & \textbf{0.514} &  \textbf{15.94} & \textbf{32.55} & \textbf{71.94} & \textbf{95.06} & \textbf{98.66} \\
% \hline
\end{tabular}
}
\end{center}
\vspace{-5mm}
\end{table}
%

\noindent \textbf{Higher accuracy normals result in more precise depth}.
We examine the performance of our DCN network using surface-normal input with and without the gravity alignment, denoted as Ours-SD+g and Ours-SD in Table~\ref{tab:betterinputs}, respectively.
%
In order to highlight the impact of the surface-normal accuracy, we evaluate the networks on the gravity-non-aligned subset of the Azure Kinect dataset, which is shown to have a significant improvement on surface-normal accuracy with the gravity alignment (see Sect.~\ref{ssec:exp_azure}).
%
Table~\ref{tab:betterinputs} illustrates that with gravity alignment, the depth accuracy increases more as compared to ones evaluated on the entire Azure Kinect dataset (see Sect.~\ref{ssec:exp_azure}).
%
However, due to the high error in some VI-SLAM point estimates, we notice the depth enrichment with gravity does not outperform other baselines such as the one without enrichment and the one without gravity on RMSE and $\delta=1.25^3$, respectively.
%
\begin{table}[h]
\caption{Better normal results in better depth \hspace{\textwidth} (Gravity-nonaligned Azure)}
\vspace{-5mm}
\label{tab:betterinputs}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|ccccc|}
\hline
 &                 &                   &                   &  $E(\hat{D}, \delta)$      &                     &  \\ \cline{3-7}
 &	RMSE $\downarrow$ & 1.05 $\uparrow$ &	1.10$\uparrow$  &	1.25$\uparrow$ &	$1.25^2 \uparrow$ &	$1.25^3 \uparrow$ \\
\hline
\hline
Ours-SD   &	0.540 & 15.58 & 31.33 & 70.81 & 93.86 & 98.11 \\
Ours-SD+g & 0.514 & 15.94 & 32.55 & 71.94 & 95.06 & \textbf{98.66} \\
Ours-Enriched 100   & \textbf{0.510}	& 20.77 & 39.64 & 76.34 & 94.34 & 98.19 \\
Ours-Enriched 100+g & 0.517 & \textbf{22.05} & \textbf{41.52} & \textbf{78.11} & \textbf{95.41} & 98.65 \\
\hline
\end{tabular}
}
\end{center}
\vspace{-3mm}
\end{table}
%
%
% \begin{table}[ht]
% \caption{Concatenation vs. Summation on Test and Generalization Sets}
% \vspace{-8mm}
% \label{table:summation_vs_concat}
% \begin{center}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|c|c|ccccc|}
% \hline
%  &                 &                   &                   &  $E(\hat{D}, \delta)$      &                     &  \\ \cline{3-7}
%  &	RMSE $\downarrow$ & 1.05 $\uparrow$ &	1.10$\uparrow$  &	1.25$\uparrow$ &	$1.25^2 \uparrow$ &	$1.25^3 \uparrow$ \\
% \hline
% \hline
% Sum (ScanNet) &	\textbf{0.260} & \textbf{51.04} & \textbf{75.30} & \textbf{93.59} &  98.11 & 99.34 \\
% Concat (ScanNet) &	0.269 & 50.95 & 75.26 & 93.23 & \textbf{98.36} &	\textbf{99.55} \\
% \hline
% Sum (Azure) &	0.990  & 15.37 & 30.39 & 65.31 & 90.90 & 95.83 \\
% Concat (Azure) & \textbf{0.639}  & \textbf{18.51} & \textbf{34.98} & \textbf{69.39} & \textbf{92.47} & \textbf{97.18} \\
% \hline
% \end{tabular}
% }
% \end{center}
% \vspace{-5mm}
% \end{table}

% \noindent \textbf{Feature concatenation improves generalization performance}.
% %
% Qiu~\etal~\cite{qiu2019deeplidar} proposed to concatenate the normal or color features with the decoder output and add the depth features (similar to a skip-connection), instead of simply concatenating color, normal, and depth features as shown in our network architecture.
% %
% Since the structure of our networks are different, we cannot replicate this approach exactly.
% %
% Instead, we first concatenate normal and color features, pass them through a convolution layer to create features of the same dimension as the depth features and then employ summation.
% %
% We train this network on ScanNet with sparse depth input.
% %
% Table~\ref{table:summation_vs_concat} provides a comparison of performance of this network (Sum) and ours (Concat) on ScanNet and Azure Kinect datasets. 
% %
% From these results, we confirm that the summation performs slightly better on ScanNet, but significantly worse on Azure Kinect and hence has less generalization capability, which is the problem we address.

\noindent \textbf{Training with depth enrichment inputs degrades cross-dataset performance}. So far, we have employed the depth enrichment method on the networks trained with VI-SLAM's sparse depth input. 
%
In Table~\ref{table:training_de_inputs}, we examine the performance of our DCN that is  \emph{trained with depth enrichment input}, denoted as Train w/ Enriched X, where X is the number of enriched samples. 
%
Note that, during the inference time, we use the same amount of enriched samples as in the training for those images that depths can be reconstructed from detected planar surface, otherwise, we use the sparse depth.
%
Due to this unavailability of plane mask in many images, there is large performance gap between networks trained with input as enriched depth and as sparse depth, suggesting that one should apply the depth enrichment technique only on a pre-trained sparse depth network.
\begin{table}[h]
\caption{Training with depth enrichment input (Azure)}
\vspace{-5mm}
\label{table:training_de_inputs}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|ccccc|}
\hline
 &                 &                   &                   &  $E(\hat{D}, \delta)$      &                     &  \\ \cline{3-7}
 &	RMSE $\downarrow$ & 1.05 $\uparrow$ &	1.10$\uparrow$  &	1.25$\uparrow$ &	$1.25^2 \uparrow$ &	$1.25^3 \uparrow$ \\
\hline
\hline
Train w/ Enriched 50   & 0.563 &	17.11 & 32.49 & 65.37 & 92.64 & 98.10 \\
Train w/ Enriched 100 & 0.562 & 17.67 & 33.56 & 68.13 & 93.57 & 98.13 \\
Train w/ Enriched 200   & 0.537 & 18.94 & 35.78 & 70.63 & 92.90 & 97.94 \\
Ours-Enriched 100 & \textbf{0.516} & \textbf{19.43} & \textbf{38.18} & \textbf{75.85} & \textbf{94.81} & \textbf{98.48} \\
\hline
\end{tabular}
}
\end{center}
\vspace{-3mm}
\end{table}

==> iros_2020_arxiv/tex/conclusions.tex <==
\section{Conclusions and Future Work}
In this paper, we introduced straightforward yet highly effective techniques to improve the generalization performance of sparse-to-dense depth completion by (i) transforming the data to a form that the network is familiar with to produce better surface normal estimates, and (ii) generating an enriched sparse depth image that significantly improves the performance both on similar scenes to the training ones and the generalization datasets collected by different devices.
%
We thoroughly evaluate multiple configurations of our approach and show the superior performance and generalization ability comparing to other state-of-the-art depth completion methods.
%
As part of the future work, we plan to incorporate the uncertainty of depth inputs to the network. 
%
Specifically, we will investigate alternative methods for enriching the sparse depth based on uncertainty instead of random sampling.
